Decoding the Protein-ligand Interactions Using Parallel Graph Neural Networks

Protein-ligand interactions (PLIs) are fundamental to biochemical research and their identification is crucial for estimating biophysical and biochemical properties for rational therapeutic design. Currently, experimental characterization of these properties is the most accurate method, however, this is very time-consuming and labor-intensive. A number of computational methods have been developed in this context but most of the existing PLI prediction heavily depends on 2D protein sequence data. Here, we present a novel parallel graph neural network (GNN) to integrate knowledge representation and reasoning for PLI prediction to perform deep learning guided by expert knowledge and informed by 3D structural data. We develop two distinct GNN architectures, GNNF is the base implementation that employs distinct featurization to enhance domain-awareness, while GNNP is a novel implementation that can predict with no prior knowledge of the intermolecular interactions. The comprehensive evaluation demonstrated that GNN can successfully capture the binary interactions between ligand and proteins 3D structure with 0.979 test accuracy for GNNF and 0.958 for GNNP for predicting activity of a protein-ligand complex. These models are further adapted for regression tasks to predict experimental binding affinities and pIC50 is crucial for drugs potency and efficacy. We achieve a Pearson correlation coefficient of 0.66 and 0.65 on experimental affinity and 0.50 and 0.51 on pIC50 with GNNF and GNNP, respectively, outperforming similar 2D sequence-based models. Our method can serve as an interpretable and explainable artificial intelligence (AI) tool for predicted activity, potency, and biophysical properties of lead candidates. To this end, we show the utility of GNNP on SARS-Cov-2 protein targets by screening a large compound library and comparing our prediction with the experimentally measured data.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> outline.tex <==
Main argument:

It would be useful to have a high-throughput method to predict the activity of a ligand with a protein pocket without knowing the protein-ligand interaction beforehand.


Demonstration:

-- comparison between the df model and split model
   -- these should be trained on the same set of keys

-- analysis of the performance of both models on different test sets split by homology of the protein
   -- test sets should have same keys for both models

-- analysis of the protein similarity between training/val/test sets

-- analysis of the protein pocket similarity within each protein

-- comparison of split model for ligands paired with the correct protein but incorrect pocket (take a pocket from a different ligand)



Images:

-- AUROC, sensitivity, specificity

Notes from Mridula:
comparison between the df model and split model - This we are already doing by reporting results in the table. We have same experiments being done for df and sp model. ( 1k, 2k, covid data, 79 targets, 96 targets e.t.c )
analysis of the performance of both models on different test sets split by homology of the protein
  -- test sets should have same keys for both models - I am not sure about this. once we have trained the model, do we need to reshuffle the entire data and split based on homology? If we want to fetch targets from test based on similarity range from training data? Jenna has shared some plots for this. That might be useful. I have a csv file which gives combination of every train and test target and the homology between them. 3.  analysis of the protein similarity between training/val/test sets - already addressed in the above point. 4.  analysis of the protein pocket similarity within each protein - I have a script for this. I will send you 5. comparison of split model for ligands paired with the correct protein but incorrect pocket (take a pocket from a different ligand) - Not doing this one

List of figures
 - Top N ranks
 - Error plots
 - homology plots
 - IC50 vs predictions for DUDE active samples - IBS activity w.r.t MPro target (GNNsp model)

Tabels
 - PDBBInd and DUDE targets and decoys per target
 - Model’s ROC, specificity and sensitivity table
 - Homology detailed table.
